Algebraic Characterization of Essential Matrices and Their Averaging in Multiview Settings

Essential matrix averaging, i.e., the task of recovering camera locations and orientations in calibrated, multiview settings, is a first step in global approaches to Euclidean structure from motion. A common approach to essential matrix averaging is to separately solve for camera orientations and subsequently for camera positions. This paper presents a novel approach that solves simultaneously for both camera orientations and positions. We offer a complete characterization of the algebraic conditions that enable a unique Euclidean reconstruction of $n$ cameras from a collection of $(^n_2)$ essential matrices. We next use these conditions to formulate essential matrix averaging as a constrained optimization problem, allowing us to recover a consistent set of essential matrices given a (possibly partial) set of measured essential matrices computed independently for pairs of images. We finally use the recovered essential matrices to determine the global positions and orientations of the $n$ cameras. We test our method on common SfM datasets, demonstrating high accuracy while maintaining efficiency and robustness, compared to existing methods.

==> TheoreticalPart_excluding_idential_ev.tex <==
%\subsection{Background}


Let $I_1, \ldots, I_n$ denote a collection of $n$ images of a static scene captured respectively by cameras $P_1,\dots,P_n$. Each camera $P_i$ is represented by a $3 \times 4$ matrix $P_i=K_i R_i^T[I,-t_i]$ where $K_{i}$ is a $3\times 3$ calibration matrix, $\bf{t}_i\in \mathbb{R}^3$ and $R_i \in SO(3)$ denote the position and orientation of $P_i$, respectively, in some global coordinate system.   We further denote $V_i=K_i^{-T}R_i^{T}$, so $P_i=V_i^{-T}[I,-{\bf t}_i]$.  Consequently, let $\bold{X}=(X,Y,Z)^T$ be a scene point in the global coordinate system. Its projection onto $I_i$ is given by ${\bf x}_i = \bold{X}_{i} / Z_i$, where $\bold{X}_{i}=(X_i, Y_i, Z_i)^T = K_{i}R_{i}^{T}(\bold{X}-{\bf t}_{i})$.  %the objective is to retrieve the $n$ positions and rotations of the cameras denoted by ${\bf t}_i \in \Real^3$ and $R_i \in SO(3)$ respectively, where $i=1\dots n$, and are defined up to a global similarity transform of the coordinates system. Let
 
%hence we can fix \(K_i=I_{3\times3}\) for all \(i\) (since if it is not the case we can multiply all the 2D points by the calibration matrix).    Let $P=(X,Y,Z)^T$ be a scene point in the global coordinate system. Its projection onto $I_i$ is given by ${\bf p}_i = P_i / Z_i$, where $P_{i}=(X_i, Y_i, Z_i)^T = R_{i}^{T}(P-{\bf t}_{i})$. We therefore associate with $I_i$ the $3 \times 4$ camera matrix $C_i=  R_i^T[I,-{\bf t}_i]$, where $I$ is a $3 \times 3$ identity matrix. 

We denote the fundamental matrix and the essential matrix between images $I_i$ and $I_j$ by $F_{ij}$ and $E_{ij}$ respectively. It was shown in \cite{sengupta2017new, arie2012global} that $E_{ij}$ and $F_{ij}$ can be written as
$$E_{ij} = R_i^T (T_i - T_j) R_j$$
$$F_{ij} = K_i^{-T} E_{ij} K_j^{-1}=V_i(T_i-T_j)V_j^T$$
where $T_i=[{\bf t}_i]_{\times}$. 


Throughout this paper we assume that all calibration matrices are known, so our work deals with solving the problem of Euclidean SfM.


The derivations in this paper adopt the definitions   ``$n$-view  fundamental matrix" and ``consistent $n$-view fundamental matrix" made in the paper \cite{kasten2018gpsfm}. We first cite these definitions, for the sake of clarity, and then define analogous definitions for the calibrated case.  In the definitions below we  denote the space of all the $3n \times 3n$ symmetric matrices by $\mathbb{S}^{3n}$.    
\begin{definition}   \label{def:mv_fundamental} 
A matrix $F \in \mathbb{S}^{3n}$, whose $3 \times 3$ blocks are denoted by $F_{ij}$, is called an {\bf n-view  fundamental matrix} if  $ \forall  i\neq j \in \{1\dots n\},$ $rank(F_{ij})=2$ and $\forall  i $  $F_{ii}=0$.
\end{definition}

\begin{definition}   \label{def:consistent_mv_fundamental} 
An $n$-view  fundamental matrix $F$ is called {\bf consistent}  if there exist camera matrices $P_1,...,P_n$ of the form $P_{i}=V_{i}^{-T}[I,\mathbf{t}_{i}]$ such that $F_{ij}=V_{i}([\mathbf{t}_{i}]_{\times}-[\mathbf{t}_{j}]_{\times})V_{j}^{T}$.
\end{definition}


\begin{definition}  \label{def:mv_essential} 
A matrix $E \in \mathbb{S}^{3n}$, whose $3 \times 3$ blocks are denoted by $E_{ij}$, is called an {\bf n-view essential  matrix} if   $\forall  i\neq j \in \{1\dots n\}$ , $rank(E_{ij})=2$, the two singular values of $E_{ij}$ are equal, and $\forall  i $ $  E_{ii}=0$.
\end{definition}

\begin{definition}
 \label{def:consistent_mv_essential}
 An $n$-view essential  matrix $E$ is called {\bf consistent} if there exist $n$ rotation matrices $\{R_i\}_{i=1}^{n}$, $n$  vectors $\{{\bf t}_i\}_{i=1}^{n}$  such that $E_{ij}= R_{i}^{T}([\mathbf{t}_{i}]_{\times}-[\mathbf{t}_{j}]_{\times})R_{j}$. \end{definition}

 
Note that any (consistent) $n$-view essential matrix is also a (consistent) $n$-view fundamental matrix. In \cite{kasten2018gpsfm}   necessary
and  sufficient conditions for the consistency of the n-view fundamental matrix were proved. The main theoretical contribution of \cite{kasten2018gpsfm} is summarized in Theorem~\ref{thm:consistent_direct}. For  the consistency of n-view essential matrix, a partial set of necessary conditions were derived in \cite{sengupta2017new}, summarized below in Theorem \ref{thm:necessary_essential}  

 


\begin{theorem}\label{thm:consistent_direct} 
 An n-view fundamental matrix $F$ is consistent with a set of $n$ cameras whose centers are not all collinear if, and only if, the following conditions hold: 
\begin{enumerate}
\item $Rank(F)=6$ and $F$ has exactly 3 positive and 3 negative eigenvalues.
\item $Rank(F_i) = 3$ for all $i =1, ..., n$, where $F_i$  is the $3 \times 3n$  $i^{th}$ block row of $F$.\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm:necessary_essential} Let $E$ be a consistent $n$-view essential matrix, associated with rotation matrices $\{R_i\}_{i=1}^n$ and camera centers $\{{\bf t}_i\}_{i=1}^n$.  $E$ satisfies the following conditions
\begin{enumerate}
\item $E$ can be formulated as $E = A + A^T$ where $A=UV^T$ and $U, V \in \Real^{3n \times 3}$
\begin{align*}
V =\left[\begin{array}{ccc}
R_{1}^T\\
\vdots\\
R_{n}^T
\end{array}\right] ~~ & ~~
U =\left[\begin{array}{c}
R_{1}^T T_{1}\\
\vdots\\
R_{n}^T T_{n}
\end{array}\right]
\end{align*}
with $T_i = [{\bf t}_i]_{\times}$ and $\sum_{i=1}^n {\bf t}_i = 0$.
\item Each column of $U$ is orthogonal to each column of $V$, i.e., $V^T U=0_{3 \times 3}$


\item rank(V)=3 

\item If not all $\{{\bf t}_i\}_{i=1}^n$ are collinear, then rank(U) and rank(A) = 3. Moreover, if the (thin) SVD of $A$ is  $A=\hat{U}\Sigma\hat{V^{T}}$, with  $\hat {U}, \hat {V} \in \Real^{3n \times 3}$ and $\Sigma \in \Real^{3 \times 3}$ then
 the (thin) SVD of $E$ is $$E = \left[\hat{U},\hat{V}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
\hat{V}^{T}\\
\hat{U}^{T}
\end{array}\right]$$
implying  rank(E) = 6.
\end{enumerate}
\end{theorem}




\subsection{Main theoretical results}
In this paper,   we derive    and prove necessary and sufficient conditions for the consistency of $n$-view essential matrices, in terms of their spectral decomposition. The conditions and the proof are presented in  Theorem \ref{consistencyThm}. These conditions, in turn, will be  used  later to formulate a constrained optimization problem and to extract the motion parameters from a consistent $n$-view essential matrix $E$ . 
\begin{theorem}\label{consistencyThm} Let $E \in \mathbb{S}^{3n}$ be a consistent $n$-view fundamental matrix with a set of $n$ cameras  whose centers are not all collinear. We denote by $\Sigma_+ ,\Sigma_- \in \mathbb{R}^{3\times3}$ the diagonal matrices with   the 3 positive and 3 negative eigenvalues of $E$, respectively. Then, the following conditions are equivalent:
\begin{enumerate}
\item $E$ is a consistent $n$-view essential matrix
\item The (thin) SVD of $E$   can be written in the form  $$E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$$
with $\hat{U}, \hat{V} \in \Real^{3n \times 3}$ such that each $3 \times 3$ block of  $\hat{V}$, $\hat{V}_i$, $i=1, \ldots, n$,  is  n-scaled rotation matrix, i.e., ${\hat V_i}=\frac{1}{\sqrt{n}} {\hat R}_i $, where ${\hat R}_i \in SO(3) $.  
We say that $\hat{V}$ is a block rotation matrix.

\item $\Sigma_+ = - \Sigma_-$ and the  (thin) spectral decomposition of $E$ is of the form $$E=[X, Y]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{-}
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]$$   such that $\sqrt{0.5}(X+Y)$ is a block rotation matrix.
\end{enumerate}
\end{theorem} 


% %\section{ Consistency Conditions  }
% 
% In this section we  state and prove our main theoretical results which gives equivalent conditions for the consistency of the $n$-view essential matrix in terms of its eigenvalues and singular values decompositions . These, in turn, will be  used  later to formulate a constrained optimization problem and to extract the motion parameters from a consistent $n$-view essential matrix $E$ . 
% 
% \uline{Notation}- Let $E\in \mathbb{S}^{3n}$ be a consistent $n$-view fundamental matrix:
% \begin{enumerate}
% \item We denote by  $\Sigma_+ ,\Sigma_- \in \mathbb{R}^{3\times3}$ the $3 \times 3$ diagonal matrices containing  the 3 positive and 3 negative eigenvalues of $E  $ respectively.
% \item We denote by $[X,Y]\in \mathbb{R}^{3n \times 6
% }$  the 6 eigenvectors of $E$ where $X\in \mathbb{R}^{3n \times 3
% }$ corresponds to 3 positive eigenvalues and $Y\in \mathbb{R}^{3n \times 3
% }$ corresponds to the 3 negative ones.
% \item  We call a matrix $A\in\mathbb{R}^{3n\times3}$ block orthogonal if each $3\times3$ block of $A$, $A_i$ is an orthogonal matrix. 
% 
% 
% \end{enumerate}
% \begin{theorem}\label{consistencyThm} Let $E \in \mathbb{S}^{3n}$ be a consistent $n$-view fundamental matrix w.r.t non-collinear camera locations, then the following conditions are equivalent:
% \begin{enumerate}
% \item $E$ is a consistent $n$-view essential matrix
% \item $\exists$ SVD of $E$   of the form  $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
% \Sigma\\
%  & \Sigma
% \end{array}\right)\left[\begin{array}{c}
%  {\hat{V}}^{T}\\
%  {\hat{U}}^{T}
% \end{array}\right]$
% such that  $\hat{V}$ is a block orthogonal matrix.
% \item It holds that $\Sigma_+ =- \Sigma_-$ and for a spectral  decomposition of $E$ associated with  the eigen vectors $X,Y$, $\exists 3\times3$ sign matrix: $I_s=\left(\begin{array}{ccc}
% \pm1 & 0 & 0 \\
% 0 & \pm1 & 0 \\
% 0 & 0 & \pm1 \\ 
% \end{array}\right)
% $ such that $X+I_s Y $ is a block orthogonal matrix.
% 
% 
% \end{theorem} 
% 
\begin{proof}


\textit{(1)$\Rightarrow$(2)}  Assume that $E$ is a consistent $n$-view essential matrix. Then, according to Thm.~\ref{thm:necessary_essential}, $E=A+A^T$ with $A=UV^T$ and $U, V \in \Real^{3n \times 3}$ with 
\begin{align*}
V =\left[\begin{array}{ccc}
R_{1}^T\\
\vdots\\
R_{n}^T
\end{array}\right] ~~ & ~~
U =\left[\begin{array}{c}
R_{1}^T T_{1}\\
\vdots\\
R_{n}^T T_{n}
\end{array}\right]
\end{align*}
where $T_i = [{\bf t}_i]_{\times}$. 
Since $A=UV^T$ and $rank(A)=3$, then $A^TA=VU^TUV$ and $A^TA \succeq 0$ with $rank(A^TA)=3$ ($A$ and $A^TA$ share the same null space). First, we construct  a spectral decomposition to $A^TA$, relying on the special properties of $U$ and $V$. We have $rank(U)=3$, and therefore $U^TU$ which is symmetric positive semi-definite matrix $3 \times 3$ matrix, is full rank. Its spectral decomposition (also svd) is of the form $U^TU = P D P^T$, where $P \in SO(3)$ (this is possible, since the spectral decomposition guarantees that $P \in O(3)$ and this can be modified by changing the sign of $P$, which flips the sign of $\text {det}(P)$ while keeping the spectral decomposition) and $D \in \Real^{3 \times 3}$ is a diagonal matrix, where the eigenvalues (singular values) of $U^TU$ forms the diagonal. This spectral decomposition yields the following decomposition 
\begin{equation}\label{eq:decomposition}
A^T A = VPDP^TV^T.
\end{equation}
Now, note that
\begin{align*}
P^TV^T VP & = P^T \begin{bmatrix}R_1 & \ldots & R_n \end{bmatrix} \begin{bmatrix}R_1^T \\ \vdots \\ R_n^T \end{bmatrix} P \\ & = P^Tn I_{3 \times 3} P=n I_{3 \times 3}. 
\end{align*}
By a simple manipulation \eqref{eq:decomposition} becomes a spectral decomposition (also svd)  
\begin{equation}\label{eq:spectral1}
 A^TA= \frac{1}{\sqrt{n}}VP(nD)P^TV^T\frac{1}{\sqrt{n}}.\end{equation}
On the other hand, the (thin) SVD of $A$ is of the form $A ={\hat U} \Sigma {\hat V}^T$, where ${\hat U}, {\hat V} \in \Real^{3n \times 3}$, $\Sigma \in \Real^{3 \times 3}$. This means that 
\begin{equation}\label{eq:spectral2}
A^TA = {\hat V} \Sigma^2 {\hat V}^T.
\end{equation} 
Due to the uniqueness of the spectral decomposition, \eqref{eq:spectral1} and \eqref{eq:spectral2} collapse to the same spectral decomposition, that is  $\frac{1}{\sqrt n} VP= {\hat V}$, which means that ${\hat V}_i = \frac{1}{\sqrt{n}} R_i^TP$. Since $R_i^T, P \in SO(3)$, then ${\hat R}_i=R_i^TP \in SO(3)$, showing that ${\hat V}$ is a block rotation matrix. The  argument derived here is true under the assumption that the 3 eigenvalues of $U^TU = \sum_{i=1}^n T_i^TT_i$ are different, residing in a descending order along the diagonal of $D$. {\textcolor{red}{Can we  move this assumption outside the theorem? }} Finally, by Thm. \ref{thm:necessary_essential}, the (thin) SVD of $E$ is 

\begin{equation}\label{eq:E_SVD}
E = \left[\hat{U},\hat{V}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
\hat{V}^{T}\\
\hat{U}^{T}
\end{array}\right].
\end{equation}
We still need to show that $\Sigma = \Sigma_+$. $E$ has three positive eigenvalues and three negative eigenvalues. Since $E$ is a symmetric matrix its singular values are equal to the absolute values of its eigenvalues. Under the assumption, claimed above, over the non-multiplicity of the singular values, which are the diagonal elements of   $\Sigma$, the structure of \eqref{eq:E_SVD} implies that $\Sigma = \Sigma_+ = |\Sigma_-|$, concluding the proof.   

 
  
 
 




\textit{(2)$\Rightarrow$(1)} Let $E$ be a consistent $n$-view fundamental matrix that satisfies condition (2). We would like to show that $E$  is a consistent $n$-view essential matrix. By condition (2) $E$ can be written as
\begin{equation}\label{eq:E_hat}
E={\hat{U}}\Sigma_+{\hat{V}^{T}}+\hat{V}\Sigma_+{\hat{U}^{T}}=\bar{{U}}\hat{V}^T+\hat{V}\bar{U^{T}}
\end{equation}
where ${\bar U}={\hat U} \Sigma_+$ with  ${\hat V}_i = \frac{1}{\sqrt n} {\hat R}_i$, ${\hat R}_i \in SO(3)$. By definition  $E_{ii}=0$, and this implies that $\bar{U}_i\hat{V}_i^T$ is a skew symmetric matrix. Using  Lemma \ref{lemma:skew},  $\bar{U}_i=\hat{V}_i {\hat T}_i $ for some skew symmetric matrix ${\hat T}_i = [{\hat {\bf t}}_i]_{\times}$. Plugging ${\bar U}_i$ and ${\hat V}_i$ in \eqref{eq:E_hat} yields 
\begin{align*}
E_{ij}&=\bar{U}_i\hat{V}_j^T+\hat{V}_i\bar{U}_j^T \\
      &= \frac{1}{n}{\hat R}_i {\hat T}_i {\hat R}_j^T - \frac{1}{n}{\hat R}_i {\hat T}_j {\hat R}_j^T \\
&=: {R_i}^T([{\bf t}_i]_{\times} - [{\bf t}_j]_{\times})R_j 
\end{align*}
where $R_i =: {\hat R}_i^T$ and  ${\bf t}_i =: \frac{1}{n} {\hat{\bf t}}_i$, concluding the proof.

\textit{(2)$\Rightarrow$(3)} Let $E$ be an $n$-view fundamental matrix which satisfies condition (2). This means that the (thin) SVD\ of $E$ can be written in the form $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$ where $\hat{V}$ is a block rotation matrix. Then, by Lemma \ref{SVDtoSPEC}, the (thin) spectral decomposition of $E$ is $E=[X, Y]\left(\begin{array}{cc}
\Sigma_{+}\\
 & -\Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]$   where $X, Y$ are the eigenvectors of $E$ with the relation \ $X = \sqrt{0.5}({\hat U}+{\hat V}) $ and $Y=\sqrt{0.5}({\hat V}-{\hat U})$. Since ${\hat V} = \sqrt{0.5} (X+Y)$, and by condition (2) ${\hat V}$  is a block rotation matrix, the claim is confirmed and also $\Sigma_- = - \Sigma_+$.

 

 \textit{(3)$\Rightarrow$(2)}   Let $E$ be a consistent $n$-view fundamental matrix satisfying condition (3), i.e.,  its  (thin) spectral decomposition is of the form $E=\left[ {X},{Y}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{-}
\end{array}\right)\left[\begin{array}{c}
 {X}^{T}\\
 {Y}^{T}
\end{array}\right]$, where $\sqrt{0.5}(X+Y)$ is a block rotation matrix. Since $\Sigma_+ = -\Sigma_-$, we can use  Lemma \ref{SVDtoSPEC}, which implies   that the (thin) SVD is of the form $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$
where ${\hat V} = \sqrt{0.5}(X+Y)$, concluding the proof.



\begin{comment}
\textit{(1)$\Rightarrow$(4)} Let $E$ be a consistent $n$-views essential matrix, by definition of consistency, $$E_{ij}=R_{i}([\mathbf{t}_{i}]_{\times}-[\mathbf{t}_{j}]_{\times})R_{j}^{T}
=[R_{i}^T(\mathbf{t}_{i}-\mathbf{t}_{j})]_{\times}R_{i}R_{j}^{T}:=T_{ij}R_{ij}$$ The above implies that each block $E_{ij}$ has equal singular values and the relative rotation satisfy that for every 3 frames $I_i,I_j,I_k$ it holds that $R_{ij}^TR_{ik}=R_jR_k=R_{jk}$ which is suffice for condition (4) to hold.\\
\textit{(4)$\Rightarrow$(1)}\ag{TBD Yoni if you can prove it easly do it if not we need to leave this section}
\end{comment}
\end{proof}


\begin{corollary} \label{EucRecon}
Euclidean reconstruction. Let $E$ be  a
consistent $n$-view essential matrix, then it is  possible to explicitly determine $R_1 \dots R_n$ and ${\bf t}_1,\ldots,{\bf t}_n$ that are consistent with respect to $E.$

\end{corollary}
\begin{proof}
The claim is justified by the following construction,
which relies on the observations  from Thm.  \ref{consistencyThm}.
\begin{enumerate}
\item Calculate the eigenvectors $X, Y$ of $E$, and  the corresponding three positive eigenvalues, $\Sigma_+$,  and three negative eigenvalues, $\Sigma_-$, respectively. 
\item  To realize condition (3), there are 8 possibilities of $\sqrt{0.5}(X+ YI_{s})$ where   $I_s=\left(\begin{array}{ccc}
\pm1 & 0 & 0 \\
0 & \pm1 & 0 \\
0 & 0 & \pm1 \\ 
\end{array}\right  )$to verify which of them is indeed a block rotation matrix.   \item  This spectral decomposition determines  directly an SVD decomposition in the form of condition (2).  $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_+\\
 & \Sigma_+
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right  ]$, where ${\hat V}$  is a block rotation matrix, i.e., ${\hat V}_i = \frac{1}{\sqrt n} {\hat R}_i$, , ${\hat R}_i \in SO(3)$.
\rb{We should explain why we cannot use SVD directly -- i.e., to avoid dealing with the multiplicities of the singular values. What happens if the eigenvalues have multiplicities?}  
\item Having the relation $E_{ij}=\hat{U}_i\Sigma_+ \hat{V}_j^T+\hat{V}_i\Sigma_+ \hat{U}_j^T$ and since $E_{ii}=0$ we get that $\hat{U}_i\Sigma_{+} \hat{V}_i^T$ is skew symmetric. We denote ${\bar U}_i={\hat U}_i \Sigma_+$ and by Lemma  \ref{lemma:skew}, it holds that ${\bar U}_i={\hat V}_i {\hat T}_i$ for some  skew symmetric ${\hat T}_i=[{\hat {\bf t}}_i]_{\times}$ \rb{So how do I determine $\hat T_i$?}
\item Therefore, 
\begin{align*}
E_{ij} & =\bar{U}_i\hat{V}_j^T+\hat{V}_i\bar{U}_j^T \\
& = \frac{1}{n}{\hat R}_i {\hat T}_i {\hat R}_j^T - \frac{1}{n}{\hat R}_i {\hat T}_j {\hat R}_j^T\\
&  = {R_i}^T([{\bf t}_i]_{\times} - [{\bf t}_j]_{\times})R_j
\end{align*}
where $R_i = {\hat R}_i^T$ and  ${\bf t}_i = \frac{1}{n} {\hat{\bf t}}_i$. \end{enumerate}
This construction  yields $\{R_i\}_{i=1}^{i=n}$ and $\{{\bf t}_i\}_{i=1}^{i=n}$ which are consistent with respect to $E$  and it is unique up to a global similarity transformation. 

\subsection{Supporting Lemmas}

\begin{comment}
\begin{lemma} \label{lemmaRotations}- Let $A=UV^T$ where $U,V$ are defined by lemma \ref{lemmaUV} eq. \eqref{UVeq} \eqref{UVeq2}
If the SVD of $A$ is $A=\hat{U}\Sigma\hat{V^{T}}$
  then $\hat{V}$ is given by $n\hat{V}=\left(\begin{array}{c}
R_{1}^{T}P\\
\vdots\\
R_{n}^{T}P
\end{array}\right)$ where $R_{i}$ is the global rotation of the i'th frame and $P$ is an orthogonal
matrix.
\end{lemma}
\begin{proof}- Let $A$ be as in lemma \ref{lemmaUV}. Lets denote $R_{3n\times3n}=\left(\begin{array}{ccc}
R_{1}^{T}\\
 & \ddots\\
 &  & R_{n}^{T}
\end{array}\right)$  and $B=R^{T}AR$. Since $R$ is a rotation matrix, every SVD of $A  $ can be transfered to an SVD of $B$ using $R$ , observing that \textbf{
\begin{align*}
B & =\left(\begin{array}{ccc}
T_{1} & \cdots & T_{1}\\
 & \ddots\\
T_{n} & \ldots & T_{n}
\end{array}\right)\\
\end{align*}
 }Next, let us denote the SVD of $B$ as $B=\bar{U_{B}}\Sigma\bar{V_{B}^{T}}$.
By definition, the right singular vectors of $B$ are the eigenvectors
of $B^{T}B$ which equal to
\begin{align*}
B^{T}B & =\left(\begin{array}{ccc}
-\sum_{i}T_{i}^{2} & \cdots & -\sum_{i}T_{i}^{2}\\
 & \ddots\\
-\sum_{i}T_{i}^{2} & \cdots & -\sum_{i}T_{i}^{2}
\end{array}\right)\\
\end{align*}
 Using the fact that $-\sum_{i}T_{i}^{2}$ is a $3\times3$ symmetric
matrix, there  exists  $3$ orthogonal vectors $P_1,P_2,P_3$ s.t 
\begin{align*}
(-\sum_{i}T_{i}^{2})P_{i} & =\lambda_{i}P_{i}\Rightarrow\\
BB^{T}\left(\begin{array}{c}
P_{i}\\
\vdots\\
P_{i}
\end{array}\right) & =\lambda_{i}\cdot n\left(\begin{array}{c}
P_{i}\\
\vdots\\
P_{i}
\end{array}\right)
\end{align*}
So if we stack $P_1,P_2,P_3\in \mathbb{R}^3$ into a matrix denoted by $P$ we have that \begin{align*}
\bar{V_{B}} & =\left(\begin{array}{c}
P\\
\vdots\\
P
\end{array}\right)_{3n\times3}\\
\end{align*}
Now since $A=\hat{U}\Sigma\hat{V^{T}}$ and $R$ is a rotation, by
uniqueness of the SVD (assuming w.l.o.g that the singular values aren't
equal \ag{w.l.o.g is not the right term, maybe we need to assume it or to state that this is an event with prob=0}) we get that
\begin{align*}
\hat{U}\Sigma\hat{V^{T}} & =A=RBR^{T}=\\
R\bar{U}_{B}\Sigma\bar{V_{B}^{T}}R^{T}
\end{align*}
 so lastly,
\begin{align*}
\hat{V} & =R\bar{V_{B}}=\\
 & \left(\begin{array}{ccc}
R_{1}^{T}\\
 & \ddots\\
 &  & R_{n}^{T}
\end{array}\right)\left(\begin{array}{c}
P\\
\vdots\\
P
\end{array}\right)=\\
 & \left(\begin{array}{c}
R_{1}^{T}P\\
\vdots\\
R_{n}^{T}P
\end{array}\right)=V\cdot P
\end{align*}
\end{proof}
\end{comment}


\begin{lemma}\label{lemma:skew} Let $A,B\in \Real^{3\times3}$ with $rank(A)=2,\,\,rank(B)=3$
and $AB^{T}$ is skew symmetric, then
$T=B^{-1}A$ is skew symmetric \cite{kasten2018gpsfm}
\end{lemma}





\begin{lemma}\label{SVDtoSPEC}- Let $E\in \mathbb{S}^{3n}$ of rank(6), and $\Sigma \in \Real^{3 \times 3} $, a diagonal matrix, with positive elements on the diagonal. Let $X, Y, U, V \in \Real^{3n \times 3}$ and we define the mapping $(X,Y) \leftrightarrow (U,V): X = \sqrt{0.5}({\hat U}+{\hat V}), Y = \sqrt{0.5}({\hat V}-{\hat U}), {\hat U} = \sqrt{0.5}(X-Y), {\hat V} = \sqrt{0.5}(X+Y)$. 

Then,

the (thin) SVD of $E$ is of the form $$E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$$   if and only if the (thin) spectral decomposition of $E$ is 
of the form 

$$E=[X, Y]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]$$ 
\end{lemma}
\begin{proof}($\Rightarrow$)      
\begin{align}\label{eq:SVD2Spec}
E &=\left[ \hat{U},\hat{V}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
 \hat{V}^{T}\\
 \hat{U}^{T}
\end{array}\right]=\hat{U}\Sigma{\hat{V}^{T}}+\hat{V}\Sigma{\hat{U}^{T}}=\nonumber \\
 & 0.5\cdot(\hat{U}+\hat{V)}\Sigma(\hat{U}+\hat{V})^{T} -0.5\cdot(\hat{V}-\hat{U)}\Sigma(\hat{V}-\hat{U})^{T}=\nonumber \\
 & 0.5\left[\hat{U}+\hat{V},\hat{V}-\hat{U}\right]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)\left[\hat{U}+\hat{V},\hat{V}-\hat{U}\right]^{T} =\nonumber \\ 
&
[X,Y]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]
\end{align}
where  $X = \sqrt{0.5}({\hat U}+{\hat V}) $ and $ Y = \sqrt{0.5}({\hat V}-{\hat U})$. Since, $ \left[\begin{array}{c}
 \hat{U}^{T}\\
 \hat{V}^{T}
\end{array}\right]\left[ \hat{U},\hat{V}\right]=I_{6 \times 6}$, it yields $ \left[\begin{array}{c}
X^{T}\\
Y^{T}
\end{array}\right]\left[ X,Y\right]=I_{6 \times 6}$, concluding that the last term in \eqref{eq:SVD2Spec} is indeed (thin) spectral decomposition of $E$.

 ($\Leftarrow$) 
\begin{align}\label{eq:spec2SVD}
E&=[X,Y]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)[X,Y]^{T} = X\Sigma X^T-Y\Sigma Y^T= \nonumber \\
&0.5(X+Y)\Sigma(X-Y)^T+0.5(X-Y)\Sigma(X+Y)^T= \nonumber\\ &0.5[X-Y,X+Y]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)[X+Y,X-Y]^T = \nonumber \\
&[{\hat U},{\hat V}]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]
\end{align}
where  ${\hat U} = \sqrt{0.5}(X-Y) $ and $ {\hat V} = \sqrt{0.5}(X+Y)$. The same argument for orthogonality works here, showing that indeed that last term in \eqref{eq:spec2SVD} is SVD of E.
\end{proof}




==> TheoreticalPart_scaled_rotations.tex <==
\subsection{Background}


Let $I_1, \ldots, I_n$ denote a collection of $n$ images of a static scene captured respectively by cameras $P_1,\dots,P_n$. Each camera $P_i$ is represented by a $3 \times 4$ matrix $P_i=K_i R_i^T[I,-t_i]$ where $K_{i}$ is a $3\times 3$ calibration matrix, $\bf{t}_i\in \mathbb{R}^3$ and $R_i \in SO(3)$ denote the position and orientation of $P_i$ in some global coordinate system.   We further denote $V_i=K_i^{-T}R_i^{T}$, so $P_i=V_i^{-T}[I,-t_i]$.  Consequently, let $\bold{X}=(X,Y,Z)^T$ be a scene point in the global coordinate system. Its projection onto $I_i$ is given by ${\bf x}_i = \bold{X}_{i} / Z_i$, where $\bold{X}_{i}=(X_i, Y_i, Z_i)^T = K_{i}R_{i}^{T}(\bold{X}-{\bf t}_{i})$.  %the objective is to retrieve the $n$ positions and rotations of the cameras denoted by ${\bf t}_i \in \Real^3$ and $R_i \in SO(3)$ respectively, where $i=1\dots n$, and are defined up to a global similarity transform of the coordinates system. Let
 
%hence we can fix \(K_i=I_{3\times3}\) for all \(i\) (since if it is not the case we can multiply all the 2D points by the calibration matrix).    Let $P=(X,Y,Z)^T$ be a scene point in the global coordinate system. Its projection onto $I_i$ is given by ${\bf p}_i = P_i / Z_i$, where $P_{i}=(X_i, Y_i, Z_i)^T = R_{i}^{T}(P-{\bf t}_{i})$. We therefore associate with $I_i$ the $3 \times 4$ camera matrix $C_i=  R_i^T[I,-{\bf t}_i]$, where $I$ is a $3 \times 3$ identity matrix. 

We denote the fundamental matrix and the essential matrix between images $I_i$ and $I_j$ by $F_{ij}$ and $E_{ij}$ respectively. It was shown in \cite{sengupta2017new, arie2012global} that $E_{ij}$ and $F_{ij}$ can be written as
$$E_{ij} = R_i^T (T_i - T_j) R_j$$
$$F_{ij} = K_i^{-T} E_{ij} K_j^{-1}=V_i(T_i-T_j)V_j^T$$
where $T_i=[{\bf t}_i]_{\times}$. 


Throughout this paper we assume that all calibration matrices are known, so our work deals with solving the problem of Euclidean SfM.


The derivations in this paper adopt the definitions   ``$n$-view  fundamental matrix" and ``consistent $n$-view fundamental matrix" made in the paper \cite{kasten2018gpsfm}. We first cite them, for the sake of clarity, and then define analogous definitions for the calibrated case.  In the definitions below we  denote the space of all the $3n \times 3n$ symmetric matrices by $\mathbb{S}^{3n}$.    
\begin{definition}   \label{def:mv_fundamental} 
A matrix $F \in \mathbb{S}^{3n}$, whose $3 \times 3$ blocks are denoted by $F_{ij}$, is called an {\bf n-view  fundamental matrix} if  $ \forall  i\neq j \in \{1\dots n\},$ $rank(F_{ij})=2$ and $\forall  i $  $F_{ii}=0$.
\end{definition}

\begin{definition}   \label{def:consistent_mv_fundamental} 
An $n$-view  fundamental matrix $F$ is called {\bf consistent}  if there exist camera matrices $P_1,...,P_n$ of the form $P_{i}=V_{i}^{-T}[I,\mathbf{t}_{i}]$ such that $F_{ij}=V_{i}([\mathbf{t}_{i}]_{\times}-[\mathbf{t}_{j}]_{\times})V_{j}^{T}$.
\end{definition}


\begin{definition}  \label{def:mv_essential} 
A matrix $E \in \mathbb{S}^{3n}$, whose $3 \times 3$ blocks are denoted by $E_{ij}$, is called an {\bf n-view essential  matrix} if   $\forall  i\neq j \in \{1\dots n\}$ , $rank(E_{ij})=2$, the two singular values of $E_{ij}$ are equal, and $\forall  i $ $  E_{ii}=0$.
\end{definition}

\begin{definition}
 \label{def:consistent_mv_essential}
 An $n$-view essential  matrix $E$ is called {\bf consistent} if there exist $n$ rotation matrices $\{R_i\}_{i=1}^{n}$, $n$  vectors $\{{\bf t}_i\}_{i=1}^{n}$  and non-zero scalars $\{ \alpha_i \}_{i=1}^n$ such that $E_{ij}= \alpha_i R_{i}^{T}([\mathbf{t}_{i}]_{\times}-[\mathbf{t}_{j}]_{\times})R_{j}\alpha_j$. \end{definition}

 
Note that any (consistent) $n$-view essential matrix is also a (consistent) $n$-view fundamental matrix. In \cite{kasten2018gpsfm}   necessary
and  sufficient conditions for the consistency of the n-view fundamental matrices were proved. The main theoretical contribution of \cite{kasten2018gpsfm} is summarized in Theorem~\ref{thm:consistent_direct}. For  the consistency of $n$-view essential matrices, a partial set of necessary conditions were derived in \cite{sengupta2017new}. However, in  \cite{sengupta2017new} the set of  $n$-view essential matrices is rather limited in the sense that the scalars $\{\alpha_i\}_{i=1}^n$  in Def. \ref{def:consistent_mv_essential} are set to 1, i.e., allowing only pure rotations.   This limitation resulted in  a relatively  complicated  optimization scheme.   In this paper, we circumvent this limitation by allowing, scaled rotations, i.e.,  any non-zero scalar, and as explained later this yields a simplified optimization scheme.   We summarize in Theorem \ref{thm:necessary_essential}  the theoretical contribution of \cite{sengupta2017new}, while extending the scope to scaled rotations.

 


\begin{theorem}\label{thm:consistent_direct} 
 An n-view fundamental matrix $F$ is consistent with a set of $n$ cameras whose centers are not all collinear if, and only if, the following conditions hold: 
\begin{enumerate}
\item $Rank(F)=6$ and $F$ has exactly 3 positive and 3 negative eigenvalues.
\item $Rank(F_i) = 3$ for all $i =1, ..., n$.
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm:necessary_essential} Let $E$ be a consistent $n$-view essential matrix, associated with rotation matrices $\{R_i\}_{i=1}^n$ and camera centers $\{{\bf t}_i\}_{i=1}^n$.  $E$ satisfies the following conditions
\begin{enumerate}
\item $E$ can be formulated as $E = A + A^T$ where $A=UV^T$ and $U, V \in \Real^{3n \times 3}$
\begin{align*}
V =\left[\begin{array}{ccc}
\alpha_1R_{1}^T\\
\vdots\\
\alpha_nR_{n}^T
\end{array}\right] ~~ & ~~
U =\left[\begin{array}{c}
\alpha_1R_{1}^T T_{1}\\
\vdots\\
\alpha_nR_{n}^T T_{n}
\end{array}\right]
\end{align*}
with $T_i = [{\bf t}_i]_{\times}$ and $\sum_{i=1}^n \alpha_i^2 {\bf t}_i = 0$.
\item Each column of $U$ is orthogonal to each column of $V$, i.e., $V^T U=0_{3 \times 3}$


\item rank(V)=3 

\item If not all $\{{\bf t}_i\}_{i=1}^n$ are collinear, then rank(U) and rank(A) = 3. Moreover, if the (thin) SVD of $A$ is  $A=\hat{U}\Sigma\hat{V^{T}}$, with  $\hat {U}, \hat {V} \in \Real^{3n \times 3}$ and $\Sigma \in \Real^{3 \times 3}$ then
 the (thin) SVD of $E$ is $$E = \left[\hat{U},\hat{V}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
\hat{V}^{T}\\
\hat{U}^{T}
\end{array}\right]$$
implying  rank(E) = 6.
\end{enumerate}
\end{theorem}




\subsection{Main theoretical results}
In this section,   we derive    and prove necessary and sufficient conditions for the consistency of $n$-view essential matrices, in terms of their spectral properties. These, in turn, will be  used  later to formulate a constrained optimization problem and to extract the motion parameters from a consistent $n$-view essential matrix $E$ . 
\begin{theorem}\label{consistencyThm} Let $E \in \mathbb{S}^{3n}$ be a consistent $n$-view fundamental matrix with a set of $n$ cameras  whose centers are not all collinear. We denote by $\Sigma_+ ,\Sigma_- \in \mathbb{R}^{3\times3}$ the diagonal matrices with   the 3 positive and 3 negative eigenvalues of $E$, respectively. The following conditions are equivalent:
\begin{enumerate}
\item $E$ is a consistent $n$-view essential matrix
\item The (thin) SVD of $E$   can be written in the form  $$E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$$
with $\hat{U}, \hat{V} \in \Real^{3n \times 3}$ such that each $3 \times 3$ block of  $\hat{V}$, $\hat{V}_i$, $i=1, \ldots, n$,  is  n-scaled rotation matrix, i.e., ${\hat V_i}=\frac{1}{\sqrt{n}} {\hat R}_i $, where ${\hat R}_i \in SO(3) $.  
We say that $\hat{V}$ is a block rotation matrix.

\item $\Sigma_+ = - \Sigma_-$ and the  (thin) spectral decomposition of $E$ is of the form $$E=[X, Y]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{-}
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]$$   such that $\sqrt{0.5}(X+Y)$ is a block rotation matrix.
\end{enumerate}
\end{theorem} 


% %\section{ Consistency Conditions  }
% 
% In this section we  state and prove our main theoretical results which gives equivalent conditions for the consistency of the $n$-view essential matrix in terms of its eigenvalues and singular values decompositions . These, in turn, will be  used  later to formulate a constrained optimization problem and to extract the motion parameters from a consistent $n$-view essential matrix $E$ . 
% 
% \uline{Notation}- Let $E\in \mathbb{S}^{3n}$ be a consistent $n$-view fundamental matrix:
% \begin{enumerate}
% \item We denote by  $\Sigma_+ ,\Sigma_- \in \mathbb{R}^{3\times3}$ the $3 \times 3$ diagonal matrices containing  the 3 positive and 3 negative eigenvalues of $E  $ respectively.
% \item We denote by $[X,Y]\in \mathbb{R}^{3n \times 6
% }$  the 6 eigenvectors of $E$ where $X\in \mathbb{R}^{3n \times 3
% }$ corresponds to 3 positive eigenvalues and $Y\in \mathbb{R}^{3n \times 3
% }$ corresponds to the 3 negative ones.
% \item  We call a matrix $A\in\mathbb{R}^{3n\times3}$ block orthogonal if each $3\times3$ block of $A$, $A_i$ is an orthogonal matrix. 
% 
% 
% \end{enumerate}
% \begin{theorem}\label{consistencyThm} Let $E \in \mathbb{S}^{3n}$ be a consistent $n$-view fundamental matrix w.r.t non-collinear camera locations, then the following conditions are equivalent:
% \begin{enumerate}
% \item $E$ is a consistent $n$-view essential matrix
% \item $\exists$ SVD of $E$   of the form  $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
% \Sigma\\
%  & \Sigma
% \end{array}\right)\left[\begin{array}{c}
%  {\hat{V}}^{T}\\
%  {\hat{U}}^{T}
% \end{array}\right]$
% such that  $\hat{V}$ is a block orthogonal matrix.
% \item It holds that $\Sigma_+ =- \Sigma_-$ and for a spectral  decomposition of $E$ associated with  the eigen vectors $X,Y$, $\exists 3\times3$ sign matrix: $I_s=\left(\begin{array}{ccc}
% \pm1 & 0 & 0 \\
% 0 & \pm1 & 0 \\
% 0 & 0 & \pm1 \\ 
% \end{array}\right)
% $ such that $X+I_s Y $ is a block orthogonal matrix.
% 
% 
% \end{theorem} 
% 
\begin{proof}


\textit{(1)$\Rightarrow$(2)}  Assume that $E$ is a consistent $n$-view essential matrix. Then, according to Thm.~\ref{thm:necessary_essential}, $E=A+A^T$ with $A=UV^T$ and $U, V \in \Real^{3n \times 3}$ with 
\begin{align*}
V =\left[\begin{array}{ccc}
R_{1}^T\\
\vdots\\
R_{n}^T
\end{array}\right] ~~ & ~~
U =\left[\begin{array}{c}
R_{1}^T T_{1}\\
\vdots\\
R_{n}^T T_{n}
\end{array}\right]
\end{align*}
where $T_i = [{\bf t}_i]_{\times}$. 
Since $A=UV^T$ and $rank(A)=3$, then $A^TA=VU^TUV$ and $A^TA \succeq 0$ with $rank(A^TA)=3$ ($A$ and $A^TA$ share the same null space). First, we construct  a spectral decomposition to $A^TA$, relying on the special properties of $U$ and $V$. We have $rank(U)=3$, and therefore $U^TU$ which is symmetric positive semi-definite matrix $3 \times 3$ matrix, is full rank. Its spectral decomposition (also SVD) is of the form $U^TU = P D P^T$, where $P \in SO(3)$ (this is possible, since the spectral decomposition guarantees that $P \in O(3)$ and this can be modified by changing the sign of $P$, which flips the sign of $\text {det}(P)$ while keeping the spectral decomposition) and $D \in \Real^{3 \times 3}$ is a diagonal matrix, where the eigenvalues (singular values) of $U^TU$ forms the diagonal. Having this spectral decomposition yields the following decomposition 
\begin{equation}\label{eq:decomposition}
A^T A = VPDP^TV^T.
\end{equation}
Now, note that
\begin{align*}
P^TV^T VP & = P^T \begin{bmatrix}R_1 & \ldots & R_n \end{bmatrix} \begin{bmatrix}R_1^T \\ \vdots \\ R_n^T \end{bmatrix} P \\ & = P^Tn I_{3 \times 3} P=n I_{3 \times 3}. 
\end{align*}
By a simple manipulation \eqref{eq:decomposition} becomes a spectral decomposition (also SVD)  
\begin{equation}\label{eq:spectral1}
 A^TA= \frac{1}{\sqrt{n}}VP(nD)P^TV^T\frac{1}{\sqrt{n}}.\end{equation}
On the other hand, the (thin) SVD of $A$ is of the form $A ={\hat U} \Sigma {\hat V}^T$, where ${\hat U}, {\hat V} \in \Real^{3n \times 3}$, $\Sigma \in \Real^{3 \times 3}$. This means that 
\begin{equation}\label{eq:spectral2}
A^TA = {\hat V} \Sigma^2 {\hat V}^T.
\end{equation} 
Due to the uniqueness of the spectral decomposition, \eqref{eq:spectral1} and \eqref{eq:spectral2} collapse to the same spectral decomposition, that is  $\frac{1}{\sqrt n} VP= {\hat V}$, which means that ${\hat V}_i = \frac{1}{\sqrt{n}} R_i^TP$. Since $R_i^T, P \in SO(3)$, then ${\hat R}_i=R_i^TP \in SO(3)$, showing that ${\hat V}$ is a block rotational matrix. The  argument derived here is true under the assumption that the 3 singular values of $A$ are different, residing in a descending order along the diagonal of $\Sigma$. {\textcolor{red}{We need to discuss it.}} Finally, by Thm. \ref{thm:necessary_essential}, the (thin) SVD of $E$ is 

\begin{equation}\label{eq:E_SVD}
E = \left[\hat{U},\hat{V}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
\hat{V}^{T}\\
\hat{U}^{T}
\end{array}\right].
\end{equation}
We still need to show that $\Sigma = \Sigma_+$. Due to Thm. \ref{thm:consistent_direct}, $E$ has three positive eigenvalues and three negative eigenvalues. Since $E$ is a symmetric matrix its singular values are equal to the absolute values of its eigenvalues. Under the assumption  over $\Sigma$, claimed above, the structure of \eqref{eq:E_SVD} implies that $\Sigma = \Sigma_+ = |\Sigma_-|$, concluding the proof.   

 
  
 
 




\textit{(2)$\Rightarrow$(1)} Let $E$ be a consistent $n$-view fundamental matrix that satisfies condition (2). We would like to show that $E$  is a consistent $n$-view essential matrix. By condition (2) $E$ can be written as
\begin{equation}\label{eq:E_hat}
E={\hat{U}}\Sigma_+{\hat{V}^{T}}+\hat{V}\Sigma_+{\hat{U}^{T}}=\bar{{U}}\hat{V}^T+\hat{V}\bar{U^{T}}
\end{equation}
where ${\bar U}={\hat U} \Sigma_+$ with  ${\hat V}_i = \frac{1}{\sqrt n} {\hat R}_i$, ${\hat R}_i \in SO(3)$. By definition  $E_{ii}=0$, and this implies that $\bar{U}_i\hat{V}_i^T$ is a skew symmetric matrix. Using  Lemma \ref{lemma:skew},  $\bar{U}_i=\hat{V}_i {\hat T}_i $ for some skew symmetric matrix ${\hat T}_i = [{\hat {\bf t}}_i]_{\times}$. Plugging ${\bar U}_i$ and ${\hat V}_i$ in \eqref{eq:E_hat} yields 
\begin{align*}
E_{ij}&=\bar{U}_i\hat{V}_j^T+\hat{V}_i\bar{U}_j^T \\
      &= \frac{1}{n}{\hat R}_i {\hat T}_i {\hat R}_j^T - \frac{1}{n}{\hat R}_i {\hat T}_j {\hat R}_j^T \\
&= {R_i}^T([{\bf t}_i]_{\times} - [{\bf t}_j]_{\times})R_j 
\end{align*}
where $R_i = {\hat R}_i^T$ and  ${\bf t}_i = \frac{1}{n} {\hat{\bf t}}_i$, concluding the proof.

\textit{(2)$\Rightarrow$(3)} Let $E$ be an $n$-view fundamental matrix which satisfies condition (2). This means that the (thin) SVD\ of $E$ can be written in the form $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$ where $\hat{V}$ is a block rotation matrix. Then, by Lemma \ref{SVDtoSPEC}, the (thin) spectral decomposition of $E$ is $E=[X, Y]\left(\begin{array}{cc}
\Sigma_{+}\\
 & -\Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]$  $E$ where $X, Y$ are the eigenvectors of $E$ with the relation \ $X = \sqrt{0.5}({\hat U}+{\hat V}) $ and $Y=\sqrt{0.5}({\hat V}-{\hat U})$. Since ${\hat V} = \sqrt{0.5} (X+Y)$, and by condition (2) ${\hat V}$  is a block rotation matrix, the claim is confirmed and also $\Sigma_- = - \Sigma_+$.

 

 \textit{(3)$\Rightarrow$(2)}   Let $E$ be a consistent $n$-view fundamental matrix satisfying condition (3), i.e.,  its  (thin) spectral decomposition is of the form $E=\left[ {X},{Y}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{-}
\end{array}\right)\left[\begin{array}{c}
 {X}^{T}\\
 {Y}^{T}
\end{array}\right]$, where $\sqrt{0.5}(X+Y)$ is a block rotation matrix. Since $\Sigma_+ = -\Sigma_-$, we can use  Lemma \ref{SVDtoSPEC}, which implies   that the (thin) SVD is of the form $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_{+}\\
 & \Sigma_{+}
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$
where ${\hat V} = \sqrt{0.5}(X+Y)$, concluding the proof.



\begin{comment}
\textit{(1)$\Rightarrow$(4)} Let $E$ be a consistent $n$-views essential matrix, by definition of consistency, $$E_{ij}=R_{i}([\mathbf{t}_{i}]_{\times}-[\mathbf{t}_{j}]_{\times})R_{j}^{T}
=[R_{i}^T(\mathbf{t}_{i}-\mathbf{t}_{j})]_{\times}R_{i}R_{j}^{T}:=T_{ij}R_{ij}$$ The above implies that each block $E_{ij}$ has equal singular values and the relative rotation satisfy that for every 3 frames $I_i,I_j,I_k$ it holds that $R_{ij}^TR_{ik}=R_jR_k=R_{jk}$ which is suffice for condition (4) to hold.\\
\textit{(4)$\Rightarrow$(1)}\ag{TBD Yoni if you can prove it easly do it if not we need to leave this section}
\end{comment}
\end{proof}


\begin{corollary} \label{EucRecon}
Euclidean reconstruction. Let $E$ be  a
consistent $n$-view essential matrix, then it is  possible to explicitly determine $R_1 \dots R_n$ and ${\bf t}_1,\ldots,{\bf t}_n$ that are consistent with respect to $E.$

\end{corollary}
\begin{proof}
The claim is justified by the following construction,
which relies on the observations  from Thm.  \ref{consistencyThm}.
\begin{enumerate}
\item Calculate the eigenvectors $X, Y$ of $E$, and  the corresponding three positive eigenvalues, $\Sigma_+$,  and three negative eigenvalues, $\Sigma_-$, respectively. 
\item  To realize condition (3), there are 8 possibilities of $\sqrt{0.5}(X+ YI_{s})$ where   $I_s=\left(\begin{array}{ccc}
\pm1 & 0 & 0 \\
0 & \pm1 & 0 \\
0 & 0 & \pm1 \\ 
\end{array}\right  )$to verify which of them is indeed a block rotation matrix.   \item  This spectral decomposition determines  directly an SVD decomposition in the form of condition (2).  $E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma_+\\
 & \Sigma_+
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right  ]$, where ${\hat V}$  is a block rotation matrix, i.e., ${\hat V}_i = \frac{1}{\sqrt n} {\hat R}_i$, , ${\hat R}_i \in SO(3)$.
\rb{We should explain why we cannot use SVD directly -- i.e., to avoid dealing with the multiplicities of the singular values. What happens if the eigenvalues have multiplicities?}  
\item Having the relation $E_{ij}=\hat{U}_i\Sigma_+ \hat{V}_j^T+\hat{V}_i\Sigma_+ \hat{U}_j^T$ and since $E_{ii}=0$ we get that $\hat{U}_i\Sigma_{+} \hat{V}_i^T$ is skew symmetric. We denote ${\bar U}_i={\hat U}_i \Sigma_+$ and by Lemma  \ref{lemma:skew}, it holds that ${\bar U}_i={\hat V}_i {\hat T}_i$ for some  skew symmetric ${\hat T}_i=[{\hat {\bf t}}_i]_{\times}$ \rb{So how do I determine $\hat T_i$?}
\item Therefore, 
\begin{equation*}
\begin{align*}
E_{ij} & =\bar{U}_i\hat{V}_j^T+\hat{V}_i\bar{U}_j^T \\
& = \frac{1}{n}{\hat R}_i {\hat T}_i {\hat R}_j^T - \frac{1}{n}{\hat R}_i {\hat T}_j {\hat R}_j^T\\
&  = {R_i}^T([{\bf t}_i]_{\times} - [{\bf t}_j]_{\times})R_j
\end{align*}
\end{equation*}
where $R_i = {\hat R}_i^T$ and  ${\bf t}_i = \frac{1}{n} {\hat{\bf t}}_i$. \end{enumerate}
This construction  yields $\{R_i\}_{i=1}^{i=n}$ and $\{{\bf t}_i\}_{i=1}^{i=n}$ which are consistent with respect to $E$  and it is unique up to a global similarity transformation. \ag{this is not trivial, we need to prove it.}{\textcolor{red}{We need to show it.

\subsection{Supporting Lemmas}





\begin{comment}
\begin{lemma} \label{lemmaRotations}- Let $A=UV^T$ where $U,V$ are defined by lemma \ref{lemmaUV} eq. \eqref{UVeq} \eqref{UVeq2}
If the SVD of $A$ is $A=\hat{U}\Sigma\hat{V^{T}}$
  then $\hat{V}$ is given by $n\hat{V}=\left(\begin{array}{c}
R_{1}^{T}P\\
\vdots\\
R_{n}^{T}P
\end{array}\right)$ where $R_{i}$ is the global rotation of the i'th frame and $P$ is an orthogonal
matrix.
\end{lemma}
\begin{proof}- Let $A$ be as in lemma \ref{lemmaUV}. Lets denote $R_{3n\times3n}=\left(\begin{array}{ccc}
R_{1}^{T}\\
 & \ddots\\
 &  & R_{n}^{T}
\end{array}\right)$  and $B=R^{T}AR$. Since $R$ is a rotation matrix, every SVD of $A  $ can be transfered to an SVD of $B$ using $R$ , observing that \textbf{
\begin{align*}
B & =\left(\begin{array}{ccc}
T_{1} & \cdots & T_{1}\\
 & \ddots\\
T_{n} & \ldots & T_{n}
\end{array}\right)\\
\end{align*}
 }Next, let us denote the SVD of $B$ as $B=\bar{U_{B}}\Sigma\bar{V_{B}^{T}}$.
By definition, the right singular vectors of $B$ are the eigenvectors
of $B^{T}B$ which equal to
\begin{align*}
B^{T}B & =\left(\begin{array}{ccc}
-\sum_{i}T_{i}^{2} & \cdots & -\sum_{i}T_{i}^{2}\\
 & \ddots\\
-\sum_{i}T_{i}^{2} & \cdots & -\sum_{i}T_{i}^{2}
\end{array}\right)\\
\end{align*}
 Using the fact that $-\sum_{i}T_{i}^{2}$ is a $3\times3$ symmetric
matrix, there  exists  $3$ orthogonal vectors $P_1,P_2,P_3$ s.t 
\begin{align*}
(-\sum_{i}T_{i}^{2})P_{i} & =\lambda_{i}P_{i}\Rightarrow\\
BB^{T}\left(\begin{array}{c}
P_{i}\\
\vdots\\
P_{i}
\end{array}\right) & =\lambda_{i}\cdot n\left(\begin{array}{c}
P_{i}\\
\vdots\\
P_{i}
\end{array}\right)
\end{align*}
So if we stack $P_1,P_2,P_3\in \mathbb{R}^3$ into a matrix denoted by $P$ we have that \begin{align*}
\bar{V_{B}} & =\left(\begin{array}{c}
P\\
\vdots\\
P
\end{array}\right)_{3n\times3}\\
\end{align*}
Now since $A=\hat{U}\Sigma\hat{V^{T}}$ and $R$ is a rotation, by
uniqueness of the SVD (assuming w.l.o.g that the singular values aren't
equal \ag{w.l.o.g is not the right term, maybe we need to assume it or to state that this is an event with prob=0}) we get that
\begin{align*}
\hat{U}\Sigma\hat{V^{T}} & =A=RBR^{T}=\\
R\bar{U}_{B}\Sigma\bar{V_{B}^{T}}R^{T}
\end{align*}
 so lastly,
\begin{align*}
\hat{V} & =R\bar{V_{B}}=\\
 & \left(\begin{array}{ccc}
R_{1}^{T}\\
 & \ddots\\
 &  & R_{n}^{T}
\end{array}\right)\left(\begin{array}{c}
P\\
\vdots\\
P
\end{array}\right)=\\
 & \left(\begin{array}{c}
R_{1}^{T}P\\
\vdots\\
R_{n}^{T}P
\end{array}\right)=V\cdot P
\end{align*}
\end{proof}
\end{comment}


\begin{lemma}\label{lemma:skew} Let $A,B\in \Real^{3\times3}$ with $rank(A)=2,\,\,rank(B)=3$
and $AB^{T}$ is skew symmetric, then
$T=B^{-1}A$ is skew symmetric \cite{kasten2018gpsfm}
\end{lemma}





\begin{lemma}\label{SVDtoSPEC}- Let $E\in \mathbb{S}^{3n}$ of rank(6), and $\Sigma \in \Real^{3 \times 3} $, a diagonal matrix, with positive elements on the diagonal. Let $X, Y, U, V \in \Real^{3n \times 3}$ and we define the mapping $(X,Y) \leftrightarrow (U,V): X = \sqrt{0.5}({\hat U}+{\hat V}), Y = \sqrt{0.5}({\hat V}-{\hat U}), {\hat U} = \sqrt{0.5}(X-Y), {\hat V} = \sqrt{0.5}(X+Y)$. 

Then,

the (thin) SVD of $E$ is of the form $$E=\left[ {\hat{U}},{\hat{V}}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]$$   if and only if the (thin) spectral decomposition of $E$ is 
of the form 

$$E=[X, Y]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]$$ 
\end{lemma}
\begin{proof}($\Rightarrow$)      
\begin{align}\label{eq:SVD2Spec}
E &=\left[ \hat{U},\hat{V}\right]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
 \hat{V}^{T}\\
 \hat{U}^{T}
\end{array}\right]=\hat{U}\Sigma{\hat{V}^{T}}+\hat{V}\Sigma{\hat{U}^{T}}=\nonumber \\
 & 0.5\cdot(\hat{U}+\hat{V)}\Sigma(\hat{U}+\hat{V})^{T} -0.5\cdot(\hat{V}-\hat{U)}\Sigma(\hat{V}-\hat{U})^{T}=\nonumber \\
 & 0.5\left[\hat{U}+\hat{V},\hat{V}-\hat{U}\right]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)\left[\hat{U}+\hat{V},\hat{V}-\hat{U}\right]^{T} =\nonumber \\ 
&
[X,Y]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)\left[\begin{array}{c}
 X^{T}\\
 Y^{T}
\end{array}\right]
\end{align}
where  $X = \sqrt{0.5}({\hat U}+{\hat V}) $ and $ Y = \sqrt{0.5}({\hat V}-{\hat U})$. Since, $ \left[\begin{array}{c}
 \hat{U}^{T}\\
 \hat{V}^{T}
\end{array}\right]\left[ \hat{U},\hat{V}\right]=I_{6 \times 6}$, it yields $ \left[\begin{array}{c}
X^{T}\\
Y^{T}
\end{array}\right]\left[ X,Y\right]=I_{6 \times 6}$, concluding that the last term in \eqref{eq:SVD2Spec} is indeed (thin) spectral decomposition of $E$.

 ($\Leftarrow$) 
\begin{align}\label{eq:spec2SVD}
E&=[X,Y]\left(\begin{array}{cc}
\Sigma\\
 & -\Sigma
\end{array}\right)[X,Y]^{T} = X\Sigma X^T-Y\Sigma Y^T= \nonumber \\
&0.5(X+Y)\Sigma(X-Y)^T+0.5(X-Y)\Sigma(X+Y)^T= \nonumber\\ &0.5[X-Y,X+Y]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)[X+Y,X-Y]^T = \nonumber \\
&[{\hat U},{\hat V}]\left(\begin{array}{cc}
\Sigma\\
 & \Sigma
\end{array}\right)\left[\begin{array}{c}
 {\hat{V}}^{T}\\
 {\hat{U}}^{T}
\end{array}\right]
\end{align}
where  ${\hat U} = \sqrt{0.5}(X-Y) $ and $ {\hat V} = \sqrt{0.5}(X+Y)$. The same argument for orthogonality works here, showing that indeed that last term in \eqref{eq:spec2SVD} is SVD of E.
\end{proof}



